Parallel Contraction Hierarchies Can Be Efficient and Scalable

Contraction Hierarchies (CH) (Geisberger et al., 2008) is one of the most widely used algorithms for shortest-path queries on road networks. Compared to Dijkstra's algorithm, CH enables orders of magnitude faster query performance through a preprocessing phase, which iteratively categorizes vertices into hierarchies and adds shortcuts. However, constructing a CH is an expensive task. Existing solutions, including parallel ones, may suffer from long construction time. Especially, in our experiments, we observe that existing parallel solutions demonstrate unsatisfactory scalability, and have performance close to sequential algorithms. We present SPoCH (Scalable Parallelization of Contraction Hierarchies), an efficient and scalable CH construction algorithm in parallel. To address the challenges in previous work, our improvements focus on both redesigning the algorithm and leveraging parallel data structures. We compare SPoCH with the state-of-the-art sequential and parallel implementations on 16 graphs of various types. Our experiments show that SPoCH achieves speedups of 11 to 68 times over the best sequential baseline and 3.8 to 41 times over the best parallel baseline in CH construction, while maintaining competitive query performance and CH graph size. We have released our code and all datasets used in this paper.

==> algorithm.tex <==
\begin{algorithm}
    \small
    \caption{Mark Contraction} \label{alg:mark}
    \SetKwFor{parForEach}{ParallelForEach}{do}{endfor}
    \KwIn{A graph $G=(V,E,w)$}
    \KwOut{A boolean sequence $contractable$}
    \parForEach{$u\in V$}{
        \If{$degree(u)\le 3$}{
            $\mbox{mark u as contractible}$ \\
            \For {$v \mbox{ is } u \mbox{'s neighbor}$}{
                \If {$degree(v) \le degree(u)$}{
                    $\mbox{mark u as uncontractible}$ \\
                }
                \ElseIf{$degree(v) = degree(u)$ and $v.priority < u.priority$}{
                    $\mbox{mark u as uncontractible}$\\
                }
            
            }
        }
    }
\end{algorithm}

\begin{algorithm}
\small
    \caption{Contracting Graph} \label{alg:contract}
    \SetKwFor{parForEach}{ParallelForEach}{do}{endfor}
    \KwIn{A graph $G=(V,E,w)$}
    \KwOut{A contracted graph $G'=(V',E',w')$ that distance between each 2 vertices remains the same}
    $layer \leftarrow 1$ \\
    $NewEdges \leftarrow []$ \\
    \parForEach {$u\in V$}{
        $u.Priority \leftarrow Rand()$ \\
        $u.layer \leftarrow \infty$
    }
    \While{$MarkContraction(G)$} {
        \parForEach {$u\in V$}{
            \If {$u \mbox{ is contractible}$}{
                \If {$degree(u) = 1$}{
                    $v \leftarrow \mbox{u's neighbor}$ \\
                }
                \ElseIf{$degree(u) = 2$}{
                    $\langle u,v_1, w_1 \rangle, \langle u,v_2, w_2\rangle \leftarrow \mbox{u's edges}$ \\
                    $\mbox{add edge} \langle v_1, v_2, w_1+w_2\rangle \mbox{ into NewEdges}$ \\
                }
                \ElseIf{$degree(u) = 3$ and $degree(\mbox{u's neighbor}) > 2$}{
                    $\langle u,v_1, w_1\rangle,\langle u,v_2, w_2\rangle,\langle u,v_3,w_3\rangle \leftarrow \mbox{u's edges}$ \\
                    $\mbox{add edges} \langle v_1,v_2, w_1+w_2\rangle \langle v_2,v_3,w_2+w_3\rangle \langle v_1,v_3,w_1+w_3\rangle \mbox{into NewEdges}$
                }
                $\mbox{mark u as contracted in graph G}$ \\
                $u.layer \leftarrow layer$
            }
        }
        $layer \leftarrow layer + 1$
    }
    $G' \leftarrow MergeEdges(G,NewEdges)$
    
\end{algorithm}

\section{Algorithm}

The Contraction algorithm will use the original graph as an input, and after the contraction,
all the vertices with degree 1,2 and 3 will be contracted while the shortest path between
each vertices will remain the same.

In this particular algorithm, we use a function $MarkContraction$ to help us find all the
vertices that can be contracted. An vertex will be marked 'Contractible' iff. 1. this
vertex has at most 3 neighbors. 2. the degree of this vertex is smaller than all the neighbors.
3. The priority number of this vertex is smaller than all the neighbors with same degree.

When a vertex is marked as contractible, it will be contracted by the algorithm \cref{alg:contract}.
This algorithm will generates new edges for the contracted graph, and mark this vertex as
contracted, and give it a layer number for unzip when calculating the single source shortest path for this contracted vertex.
The new edges will be put into a hash bag $NewEdges$ using the source vertex as an index.
These edges will be treated as already in this graph $G$, and will be accessed by  

Whenever a vertex is marked as contracted, we consider this vertex is removed from the
graph in this contracting procedure. Although the edges will be still stored inside the graph G,
the algorithm will ignore them when calculating the degrees and 
comparing contracting priority of the remaining vertices.

After all the contractible vertices are solved, the algorithm will generates a new graph $G'$ to
by combining the edges of the original graph $G$ and all the edges stored inside the hashbag.
In the graph $G'$, the contracted vertices will have a positive layer value, while the 
remaining vertices will have a infinity layer value. When running Shortest Path algorithm 
on this graph $G'$, all the edges with contracted source will be considered directed,
and the direction is from the vertex with lower layer to vertex with higher layer.
After all the vertices with non-infinity layer value are relaxed in SSSP, we can run a
decompress layer on the remaining graph. Since the vertices with same layer value will
not affect each other, we can solve this decompress in parallel.
\begin{theorem}
    For each layer, at most 1 vertex will appear in the SSSP algorithm before decontraction.
\end{theorem}

\begin{proof}
    Consider the last contracted layer in the contracted graph, it can only have 1 vertex.
    So if the SSSP starts from this vertex, the theorem holds.

    Then, if last k layer holds the theorem, consider a source from the last k-1 layer.
    The 2 directed edge cannot targeting 2 vertices in the same layer k', since we added 
    an edge between these 2 vertices in the contracting phase. So, starting from this source, 
    at most 1 vertex in the kth layer will be added, and the vertex in the shallower layer will 
    be directly pointed by the other vertex. Then the following steps will holds the theorem,
    since the problem has been transformed into a SSSP problem in the k'th layer.

    Thus, the theorem holds.
\end{proof}


==> algorithms_comparison_table.tex <==
\begin{table*}
  \small
  \centering
  \begin{tabular}{rc|cccc|cccc|ccccc|}
    \multicolumn{2}{r|}{\multirow{2}[0]{*}{\textbf{Graph}}} & \multicolumn{4}{c|}{\textbf{Road}} & \multicolumn{4}{c|}{\textbf{Synthetic}} & \multicolumn{5}{c|}{\textbf{k-NN}} \\
    \multicolumn{2}{r|}{} & \textbf{EU} & \textbf{NA} & \textbf{AS} & \textbf{AF} & \textbf{TRCE} & \textbf{BUB} & \textbf{CHN7} & \textbf{CHN8} & \textbf{CH2} & \textbf{CH5} & \textbf{GL2} & \textbf{GL5} & \textbf{GL10} \\
    \multicolumn{2}{c|}{\textbf{\#vertices}} & 130,655,972 & 86,951,513 & 95,735,401 & 33,493,259 & 16,002,413 & 21,198,119 & 10,000,000 & 100,000,000 & 4,208,261 & 4,208,261 & 24,876,978 & 24,876,978 & 24,876,978 \\
    \multicolumn{2}{c|}{\textbf{\#edges}} & 168,541,220 & 112,869,708 & 122,836,037 & 44,773,338 & 47,997,626 & 63,580,358 & 9,999,999 & 99,999,999 & 8,416,522 & 21,041,305 & 49,753,956 & 124,384,890 & 248,769,780 \\
    \midrule
    \multicolumn{1}{r}{\multirow{4}[2]{*}{\textbf{\#edges}}} & \textbf{OURS} & 291,634,603 & 194,651,812 & 210,917,585 & 77,317,472 & 132,524,818 & 175,442,512 & 19,999,891 & 199,999,859 & 10,474,907 & 61,221,260 & 55,677,004 & 152,013,202 & 322,959,798 \\
    & \textbf{RK} & \textit{298,013,106} & \textit{197,984,621} & \textit{216,069,398} & \textit{79,158,768} & \textit{131,974,849} & \textit{174,462,657} & \textit{19,999,942} & \textit{199,999,935} & \textit{10,514,043} & \textit{52,997,166} & \textit{56,429,191} & \textit{147,182,937} & \textit{295,247,166} \\
    & \textbf{CC} & 300,867,980 & 201,063,082 & 218,803,957 & 79,724,230 & 132,090,078 & 174,420,738 & 19,999,945 & 199,999,936 & 10,608,743 & 70,997,370 & 57,310,464 & 155,481,962 & 339,610,716 \\
    & \textbf{\PHAST} & \textcolor[rgb]{ 1, 0, 0}{\textbf{TBD}} & \textcolor[rgb]{ 1, 0, 0}{\textbf{TBD}} & \textcolor[rgb]{ 1, 0, 0}{\textbf{TBD}} & \textcolor[rgb]{ 1, 0, 0}{\textbf{TBD}} & \textcolor[rgb]{ 1, 0, 0}{\textbf{TBD}} & \textcolor[rgb]{ 1, 0, 0}{\textbf{TBD}} & \textcolor[rgb]{ 1, 0, 0}{\textbf{TBD}} & \textcolor[rgb]{ 1, 0, 0}{\textbf{TBD}} & \textcolor[rgb]{ 1, 0, 0}{\textbf{TBD}} & \textcolor[rgb]{ 1, 0, 0}{\textbf{TBD}} & \textcolor[rgb]{ 1, 0, 0}{\textbf{TBD}} & \textcolor[rgb]{ 1, 0, 0}{\textbf{TBD}} & \textcolor[rgb]{ 1, 0, 0}{\textbf{TBD}} \\
    \midrule
    \multicolumn{1}{r}{\multirow{6}[2]{*}{\textbf{build time}}} & \textbf{OURS} & 46.85 & 31.39 & 33.49 & 10.91 & 31.79 & 43.87 & 2.28 & 18.55 & 1.37 & 110.18 & 4.90 & 13.60 & 46.13 \\
    & \textbf{RK} & 3,783.45 & 2,466.09 & 2,619.13 & 465.94 & 1,764.70 & 2,509.31 & 38.71 & 848.45 & 15.46 & 14,047.76 & 108.20 & 716.19 & 4,174.69 \\
    & \textbf{CC} & 2,121.35 & 1,527.47 & 1,547.93 & 334.03 & 1,218.12 & 1,679.83 & 18.97 & 217.77 & 11.04 & 4,736.59 & 83.30 & 453.36 & 2,626.93 \\
    & \textbf{\PHAST} & \textcolor[rgb]{ 1, 0, 0}{\textbf{TBD}} & \textcolor[rgb]{ 1, 0, 0}{\textbf{TBD}} & \textcolor[rgb]{ 1, 0, 0}{\textbf{TBD}} & \textcolor[rgb]{ 1, 0, 0}{\textbf{TBD}} & \textcolor[rgb]{ 1, 0, 0}{\textbf{TBD}} & \textcolor[rgb]{ 1, 0, 0}{\textbf{TBD}} & \textcolor[rgb]{ 1, 0, 0}{\textbf{TBD}} & \textcolor[rgb]{ 1, 0, 0}{\textbf{TBD}} & \textcolor[rgb]{ 1, 0, 0}{\textbf{TBD}} & \textcolor[rgb]{ 1, 0, 0}{\textbf{TBD}} & \textcolor[rgb]{ 1, 0, 0}{\textbf{TBD}} & \textcolor[rgb]{ 1, 0, 0}{\textbf{TBD}} & \textcolor[rgb]{ 1, 0, 0}{\textbf{TBD}} \\
    & \textbf{OURS\_seq} & 2,233.00 & 1,611.93 & 1,617.03 & 457.30 & 2,037.80 & 2,970.35 & 71.36 & 821.81 & 33.06 & 7,892.52 & 162.65 & 653.27 & 2,893.10 \\
    & \textbf{CC\_seq} & 3,573.98 & 2,907.06 & 2,604.48 & 552.56 & 3,657.55 & \textcolor[rgb]{ 1, 0, 0}{\textbf{-}} & 35.12 & 422.57 & 20.49 & \textcolor[rgb]{ 1, 0, 0}{\textbf{TBD}} & 132.54 & \textcolor[rgb]{ 1, 0, 0}{\textbf{TBD}} & \textcolor[rgb]{ 1, 0, 0}{\textbf{TBD}} \\
    \midrule
    \multicolumn{1}{r}{\multirow{4}[2]{*}{\textbf{\#query\newline{}iterations}}} & \textbf{OURS} & 754.59 & 492.07 & 270.97 & 101.94 & 1,821.89 & 1,631.49 & 24.79 & 28.88 & 8.91 & 844.20 & 6.10 & 36.39 & 124.74 \\
    & \textbf{RK} & 544.74 & 457.50 & 260.20 & 103.52 & 1,532.63 & 1,410.78 & 24.42 & 29.92 & 9.03 & 795.55 & 6.21 & 34.08 & 107.14 \\
    & \textbf{CC} & 1,207.39 & 951.05 & 492.89 & 201.09 & 2,668.13 & 2,432.69 & 25.12 & 28.94 & 9.07 & 1,938.75 & 6.49 & 56.14 & 265.50 \\
    & \textbf{\PHAST} & \textcolor[rgb]{ 1, 0, 0}{\textbf{TBD}} & \textcolor[rgb]{ 1, 0, 0}{\textbf{TBD}} & \textcolor[rgb]{ 1, 0, 0}{\textbf{TBD}} & \textcolor[rgb]{ 1, 0, 0}{\textbf{TBD}} & \textcolor[rgb]{ 1, 0, 0}{\textbf{TBD}} & \textcolor[rgb]{ 1, 0, 0}{\textbf{TBD}} & \textcolor[rgb]{ 1, 0, 0}{\textbf{TBD}} & \textcolor[rgb]{ 1, 0, 0}{\textbf{TBD}} & \textcolor[rgb]{ 1, 0, 0}{\textbf{TBD}} & \textcolor[rgb]{ 1, 0, 0}{\textbf{TBD}} & \textcolor[rgb]{ 1, 0, 0}{\textbf{TBD}} & \textcolor[rgb]{ 1, 0, 0}{\textbf{TBD}} & \textcolor[rgb]{ 1, 0, 0}{\textbf{TBD}} \\
    \midrule
    \multicolumn{1}{r}{\multirow{4}[1]{*}{\textbf{query\newline{}time(us)}}} & \textbf{OURS} & 191.39 & 133.36 & 81.63 & 28.77 & 537.58 & 461.91 & 7.38 & 10.42 & 3.89 & 291.84 & 3.82 & 15.67 & 49.08 \\
    & \textbf{RK} & 113.90 & 99.28 & 60.23 & 19.25 & 367.05 & 324.69 & 5.90 & 13.97 & 2.74 & 200.10 & 1.81 & 7.63 & 25.04 \\
    & \textbf{CC} & 476.95 & 391.48 & 213.08 & 75.68 & 1,053.34 & 982.98 & 9.64 & 17.08 & 3.43 & 840.80 & 4.01 & 25.05 & 114.95 \\
    & \textbf{\PHAST} & \textcolor[rgb]{ 1, 0, 0}{\textbf{TBD}} & \textcolor[rgb]{ 1, 0, 0}{\textbf{TBD}} & \textcolor[rgb]{ 1, 0, 0}{\textbf{TBD}} & \textcolor[rgb]{ 1, 0, 0}{\textbf{TBD}} & \textcolor[rgb]{ 1, 0, 0}{\textbf{TBD}} & \textcolor[rgb]{ 1, 0, 0}{\textbf{TBD}} & \textcolor[rgb]{ 1, 0, 0}{\textbf{TBD}} & \textcolor[rgb]{ 1, 0, 0}{\textbf{TBD}} & \textcolor[rgb]{ 1, 0, 0}{\textbf{TBD}} & \textcolor[rgb]{ 1, 0, 0}{\textbf{TBD}} & \textcolor[rgb]{ 1, 0, 0}{\textbf{TBD}} & \textcolor[rgb]{ 1, 0, 0}{\textbf{TBD}} & \textcolor[rgb]{ 1, 0, 0}{\textbf{TBD}} \\
    \end{tabular}%
\end{table*}

==> ch-algorithms-comparison-table-all.tex <==
% Table generated by Excel2LaTeX from sheet 'Final_all_algorithms_comparison'
\begin{table*}[htbp]
  \small
  \centering
    \begin{tabular}{ccc|cccc|cccc|ccccc|}
    \multicolumn{3}{c|}{\multirow{2}[0]{*}{\textbf{Graph}}} & \multicolumn{4}{c|}{\textbf{Road}} & \multicolumn{4}{c|}{\textbf{Synthetic}} & \multicolumn{5}{c|}{\textbf{$k$-NN}} \\
    \multicolumn{3}{c|}{} & \textbf{AF} & \textbf{NA} & \textbf{AS} & \textbf{EU} & \textbf{TRCE} & \textbf{BUB} & \textbf{CHN7} & \textbf{CHN8} & \textbf{CH2} & \textbf{CH5} & \textbf{GL2} & \textbf{GL5} & \textbf{GL10} \\
    \multicolumn{3}{c|}{\textbf{\# vertices}} & 33.5M & 87.0M & 95.7M & 131M  & 16.0M & 21.2M & 10.0M & 100M  & 4.21M & 4.21M & 24.9M & 24.9M & 24.9M \\
    \multicolumn{3}{c|}{\textbf{\# edges}} & 44.8M & 113M  & 123M  & 169M  & 48.0M & 63.6M & 10.0M & 100M  & 8.42M & 21.0M & 49.8M & 124M  & 249M \\
    \midrule
    \multicolumn{1}{c}{\multirow{13}[3]{*}{\begin{sideways}\textbf{Build}\end{sideways}}} & \multicolumn{1}{c}{\multirow{8}[2]{*}{\begin{sideways}\textbf{build time (s)}\end{sideways}}} & \textbf{*\oursysTab} & \underline{\textbf{7.32}} & \underline{\textbf{23.1}} & \underline{\textbf{23.5}} & \underline{\textbf{32.9}} & \underline{\textbf{27.2}} & \underline{\textbf{38.8}} & \underline{\textbf{1.87}} & \underline{\textbf{15.2}} & \underline{\textbf{0.89}} & \underline{\textbf{107}} & \underline{\textbf{3.00}} & \underline{\textbf{9.67}} & \underline{\textbf{41.1}} \\
          &       & \textbf{*OSRM} & 60.0  & 307   & 286   & 521   & 218   & 292   & 6.77  & 71.2  & 4.38  & 28028 & 30.7  & 103   & 391 \\
          &       & \textbf{*CC-8} & 334   & 1527  & 1548  & 2121  & 1218  & 1680  & 19.0  & 218   & 11.0  & 4737  & 83.3  & 453   & 2627 \\
          &       & \textbf{RK} & 466   & 2466  & 2619  & 3783  & 1765  & 2509  & 38.7  & 848   & 15.5  & 14048 & 108   & 716   & 4175 \\
          &       & \textbf{Phast} & 287   & 1341  & 1421  & 1865  & 1470  & 2053  & 23.5  & 285   & 9.20  & 11361 & 46.0  & 373   & 2388 \\
          &       & \textbf{\oursysTab-seq} & 386   & 1365  & 1354  & 1847  & 1816  & 2620  & 65.4  & 751   & 26.1  & 7454  & 125   & 545   & 2676 \\
          &       & \textbf{OSRM-seq} & 503   & 3246  & 2839  & 4101  & 3817  & 5273  & 34.4  & 390   & 18.3  & T.O.  & 82.4  & 1062  & 12082 \\
          &       & \textbf{CC-seq} & 553   & 2907  & 2604  & 3574  & 3658  & 5002  & 35.1  & 423   & 20.5  & 17268 & 133   & 812   & 6855 \\
\cmidrule{2-16}          & \multicolumn{1}{c}{\multirow{5}[1]{*}{\begin{sideways}\textbf{$\boldsymbol{|E_{CH}|}$}\end{sideways}}} & \textbf{*\oursysTab} & 78.3M & 197M  & 214M  & 295M  & 134M  & 177M  & 20.0M & 200M  & 10.6M & 61.4M & 56.0M & 152M  & 323M \\
          &       & \textbf{*OSRM} & \underline{\textbf{73.4M}} & \underline{\textbf{186M}} & \underline{\textbf{200M}} & \underline{\textbf{279M}} & \underline{\textbf{121M}} & \underline{\textbf{160M}} & \underline{\textbf{20.0M}} & \underline{\textbf{200M}} & \underline{\textbf{9.70M}} & \underline{\textbf{50.0M}} & \underline{\textbf{52.7M}} & \underline{\textbf{140M}} & \underline{\textbf{285M}} \\
          &       & \textbf{*CC-8} & 79.7M & 201M  & 219M  & 301M  & 132M  & 174M  & 20.0M & 200M  & 10.6M & 71.0M & 57.3M & 155M  & 340M \\
          &       & \textbf{RK} & 79.2M & 198M  & 216M  & 298M  & 132M  & 174M  & 20.0M & 200M  & 10.5M & 53.0M & 56.4M & 147M  & 295M \\
          &       & \textbf{Phast} & 78.2M & 199M  & 215M  & 298M  & 126M  & 166M  & 20.0M & 200M  & 10.7M & 52.0M & 60.5M & 145M  & 292M \\
    \midrule
    \multicolumn{1}{c}{\multirow{10}[2]{*}{\begin{sideways}\textbf{Query}\end{sideways}}} & \multicolumn{1}{c}{\multirow{5}[1]{*}{\begin{sideways}\textbf{time ($\mu$s)}\end{sideways}}} & \textbf{*\oursysTab} & 18.0  & 101   & 62.3  & 172   & 421   & 514   & 5.65  & 7.39  & 3.50  & 253   & 1.81  & 10.5  & 34.0 \\
          &       & \textbf{*OSRM} & 28.7  & 163   & 97.6  & 223   & 454   & 512   & 7.94  & 9.74  & 3.84  & 325   & 2.20  & 12.5  & 39.0 \\
          &       & \textbf{*CC-8} & 48.1  & 317   & 190   & 424   & 910   & 1010  & 7.60  & 9.07  & 3.33  & 783   & 2.11  & 17.2  & 85.2 \\
          &       & \textbf{RK} & \underline{\textbf{13.6}} & \underline{\textbf{79.1}} & \underline{\textbf{47.9}} & \underline{\textbf{102}} & \underline{\textbf{292}} & \underline{\textbf{337}} & \underline{\textbf{4.93}} & \underline{\textbf{6.33}} & \underline{\textbf{2.69}} & \underline{\textbf{176}} & \underline{\textbf{1.52}} & \underline{\textbf{6.25}} & \underline{\textbf{19.0}} \\
          &       & \textbf{Phast} & 26.7  & 138   & 84.4  & 169   & 430   & 482   & 7.73  & 9.23  & 4.09  & 278   & 2.37  & 11.8  & 33.5 \\
\cmidrule{2-16}          & \multicolumn{1}{r}{\multirow{5}[1]{*}{\begin{sideways}\textbf{\#vertices}\end{sideways}}} & \textbf{*\oursysTab} & 82.7  & 462   & 275   & 776   & 1627  & 1902  & 24.9  & 29.1  & \underline{\textbf{9.73}} & 861   & 6.34  & 34.2  & 111 \\
          &       & \textbf{*OSRM} & 96.0  & 537   & 310   & 687   & 1449  & 1616  & 25.2  & 28.9  & 11.5  & 1060  & 6.77  & 35.7  & 113 \\
          &       & \textbf{*CC-8} & 168   & 931   & 553   & 1192  & 2432  & 2739  & 25.0  & 28.6  & 10.1  & 1912  & 6.49  & 53.7  & 257 \\
          &       & \textbf{RK} & \underline{\textbf{81.8}} & \underline{\textbf{426}} & \underline{\textbf{264}} & \underline{\textbf{542}} & 1398  & \underline{\textbf{1565}} & \underline{\textbf{24.7}} & \underline{\textbf{28.6}} & 9.93  & \underline{\textbf{800}} & \underline{\textbf{6.29}} & \underline{\textbf{31.7}} & \underline{\textbf{97.8}} \\
          &       & \textbf{Phast} & 83.1  & 467   & 256   & 556   & \underline{\textbf{1386}} & 1566  & 27.0  & 30.3  & 12.7  & 910   & 7.11  & 34.0  & 97.0 \\
    \end{tabular}%
    \caption{\small \textbf{Comparison of the performance of various contraction hierarchies implementations across three representative types of graphs,
    including build time (in seconds), number of edges in the contraction hierarchies, number of scanned vertices in the s-t query and s-t query time (in microseconds).}
    Asterisks (*) are placed to the left of the algorithm names to indicate that they are parallel implementations.
    ``-seq'' means their running time on one core. 
    T.O. means timeout.}
  \label{tab:maintable}%
\end{table*}%

% Table generated by Excel2LaTeX from sheet 'algo_tot_comparison'
%$\boldsymbol{|E_{CH}|}$
%\begin{tabular}{ccc|cccc|cccc|ccccc|}
%\multicolumn{3}{c|}
%time($\mu$s)


==> ch-algorithms-comparison-table.tex <==
% Table generated by Excel2LaTeX from sheet 'Final_all_algorithms_comparison'
\begin{table*}[htbp]
  \small
  \centering
  \vspace{-.5em}
    \begin{tabular}{cl|cccc|cccc|ccccc}
    \multicolumn{2}{c|}{\multirow{2}[0]{*}{\textbf{Graph}}} & \multicolumn{4}{c|}{\textbf{Road}} & \multicolumn{4}{c|}{\textbf{Synthetic}} & \multicolumn{5}{c}{\textbf{$k$-NN}} \\
    \multicolumn{2}{c|}{} & \textbf{AF} & \textbf{NA} & \textbf{AS} & \textbf{EU} & \textbf{TRCE} & \textbf{BUB} & \textbf{CHN7} & \textbf{CHN8} & \textbf{CH2} & \textbf{CH5} & \textbf{GL2} & \textbf{GL5} & \textbf{GL10} \\
    \multicolumn{2}{c|}{\textbf{\# vertices}} & 33.5M & 87.0M & 95.7M & 131M  & 16.0M & 21.2M & 10.0M & 100M  & 4.21M & 4.21M & 24.9M & 24.9M & 24.9M \\
    \multicolumn{2}{c|}{\textbf{\# edges}} & 44.8M & 113M  & 123M  & 169M  & 48.0M & 63.6M & 10.0M & 100M  & 8.42M & 21.0M & 49.8M & 124M  & 249M \\
    \midrule
    \multirow{8}[1]{*}{\begin{sideways}\textbf{Build (s)}\end{sideways}} &  \textbf{\oursysTab*} & \underline{\textbf{7.32}} & \underline{\textbf{23.1}} & \underline{\textbf{23.5}} & \underline{\textbf{32.9}} & \underline{\textbf{27.2}} & \underline{\textbf{38.8}} & \underline{\textbf{1.87}} & \underline{\textbf{15.2}} & \underline{\textbf{0.89}} & \underline{\textbf{107}} & \underline{\textbf{3.00}} & \underline{\textbf{9.67}} & \underline{\textbf{41.1}} \\
        & \textbf{\OSRM*} & 60.0  & 307   & 286   & 521   & 218   & 292   & 6.77  & 71.2  & 4.38  & 28028 & 30.7  & 103   & 391 \\
          & \textbf{\CC*} & 334   & 1527  & 1548  & 2121  & 1218  & 1680  & 19.0  & 218   & 11.0  & 4737  & 83.3  & 453   & 2627 \\
          & \textbf{\RK} & 466   & 2466  & 2619  & 3783  & 1765  & 2509  & 38.7  & 848   & 15.5  & 14048 & 108   & 716   & 4175 \\
          & \textbf{\PHAST} & 287   & 1341  & 1421  & 1865  & 1470  & 2053  & 23.5  & 285   & 9.20  & 11361 & 46.0  & 373   & 2388 \\
          & \textbf{\oursysTab-seq} & 386   & 1365  & 1354  & 1847  & 1816  & 2620  & 65.4  & 751   & 26.1  & 7454  & 125   & 545   & 2676 \\
          & \textbf{\OSRM-seq} & 503   & 3246  & 2839  & 4101  & 3817  & 5273  & 34.4  & 390   & 18.3  & >30000  & 82.4  & 1062  & 12082 \\
          & \textbf{\CC-seq} & 553   & 2907  & 2604  & 3574  & 3658  & 5002  & 35.1  & 423   & 20.5  & 17268 & 133   & 812   & 6855 \\
    \midrule
    \multirow{5}[1]{*}{\begin{sideways}\textbf{Query ($\mu$s)}\end{sideways}} & \textbf{\oursysTab*} & 18.0  & 101   & 62.3  & 172   & 421   & 514   & 5.65  & 7.39  & 3.50  & 253   & 1.81  & 10.5  & 34.0 \\
              & \textbf{\OSRM*} & 28.7  & 163   & 97.6  & 223   & 454   & 512   & 7.94  & 9.74  & 3.84  & 325   & 2.20  & 12.5  & 39.0 \\
              & \textbf{\CC*} & 48.1  & 317   & 190   & 424   & 910   & 1010  & 7.60  & 9.07  & 3.33  & 783   & 2.11  & 17.2  & 85.2 \\
              & \textbf{\RK} & \underline{\textbf{13.6}} & \underline{\textbf{79.1}} & \underline{\textbf{47.9}} & \underline{\textbf{102}} & \underline{\textbf{292}} & \underline{\textbf{337}} & \underline{\textbf{4.93}} & \underline{\textbf{6.33}} & \underline{\textbf{2.69}} & \underline{\textbf{176}} & \underline{\textbf{1.52}} & \underline{\textbf{6.25}} & \underline{\textbf{19.0}} \\
              & \textbf{\PHAST} & 26.7  & 138   & 84.4  & 169   & 430   & 482   & 7.73  & 9.23  & 4.09  & 278   & 2.37  & 11.8  & 33.5 \\
    \end{tabular}%
    \caption{\textbf{Comparison of build time (in seconds) and query time (in microseconds) for all tested implementations across all graphs.}
    ``\oursysTab'' $=$ our algorithm.
    ``\OSRM'' $=$ Open Source Routing Machine~\cite{luxen2011real}.
    ``\CC'' $=$ CH-Constructor~\cite{chconstructor2024code}.
    ``\RK'' $=$ RoutingKit~\cite{dibbelt2016customizable}.
    ``\PHAST'' $=$ PHAST~\cite{delling2013phast}.
    %``T.O.'' $=$ timeout.
    Implementations with asterisks (*) are parallel,
    and their sequential running times (with suffices ``-seq'') are also included in the table.
    We report the parallel running time of \CC{} using eight threads,
    as this configuration yields the best performance due to its limited scalability.
}
\label{tab:ch_algo_cmp}%
  \vspace{-.5em}
\end{table*}%


==> figures/fig-ie_list.tex <==
\begin{figure}
  \centering
  \includegraphics[width=\columnwidth]{figures/ie_list_new.pdf}
  \caption{\small \textbf{An illustration of (a) path graph contraction procedure and (b) eventual outcome.  } (a):
  (b):
  }\label{fig:ie_list_new}
\end{figure}

==> figures/fig-pch.tex <==
\hide{
\begin{figure}
  \centering
  \includegraphics[width=\columnwidth]{figures/Parallel-Contraction-Hierarchies.pdf}
  \caption{\textbf{Illustration for the Parallel Construction of Contraction Hierarchies.}
  See~\cref{fig:ch} for the sequential construction.
  In each round, a vertex $v$ can be contracted in parallel if $\priority[v] < \priority[u]$ for $u\in \n(v)$.
  Here we assume the scores are unchanged and they are ordered by the vertex ids.
  }\label{fig:pch}
\end{figure}
}
\begin{figure}
  \centering
  \includegraphics[width=\columnwidth]{figures/Parallel_CH_compact.pdf}
  \caption{\textbf{Illustration for the Parallel Construction of Contraction Hierarchies.}
  See~\cref{fig:ch} for the sequential construction.
  In each round, a vertex $v$ can be contracted in parallel if $\priority[v] < \priority[u]$ for $u\in \n(v)$.
  Here we assume the scores are unchanged and they are ordered by the vertex ids.
  }\label{fig:pch}
\end{figure}

==> framework.tex <==
\begin{algorithm}[t]
    \small
    \caption{Stepping on Contracting Graph} \label{alg:SSSP}
    \SetKwFor{parForEach}{ParallelForEach}{do}{endfor}
\KwIn{A graph $G=(V,E,w)$ and a source node $s$.}
\KwOut{The graph distances $d(\cdot)$ from $s$.}
    \vspace{0.5em}
%$S_0\leftarrow \{s\}$\\
\DontPrintSemicolon
$\delta[\cdot]\leftarrow +\infty$, associate $\delta$ to $Q\in \mathbb{P}\mathbb{Q} $\\
$\delta[s]\leftarrow 0$, $Q.lazyinsert{}(s)$\\
$SSSP(G, s)$ \\
$layer \leftarrow \mbox{maximum non-infinity layer in V}$ \\
\While{$layer > 0$}{
    \parForEach{$u\in V$ and $u.layer = layer$}{
        $\delta[u] = min_{v\mbox{ is u's neighbor}}(\delta[v]+w(u,v))$
    }
    $layer \leftarrow layer - 1$
}
\Return {$\delta(\cdot)$}\\[.25em]
\end{algorithm} 

==> graph-details.tex <==
\begin{table}[h]
  \centering
    \begin{tabular}{ccc|cccc}
    \multirow{2}[1]{*}{\textbf{Graph}} & \multirow{2}[1]{*}{\textbf{\#V(M)}} & \multirow{2}[1]{*}{\textbf{\#E(M)}} & \multicolumn{4}{c}{\textbf{\#CH\_edges}} \\
          &       &       & \textbf{OURS(M)} & \textbf{RK(M)} & \textbf{CC(M)} & \textbf{Phast} \\
    \midrule
    \textbf{EU} & 131   & 169   & 292   & \textit{298} & 301   & \textcolor[rgb]{ 1,  0,  0}{\textbf{TBD}} \\
    \textbf{NA} & 87    & 113   & 195   & \textit{198} & 201   & \textcolor[rgb]{ 1,  0,  0}{\textbf{TBD}} \\
    \textbf{AS} & 96    & 123   & 211   & \textit{216} & 219   & \textcolor[rgb]{ 1,  0,  0}{\textbf{TBD}} \\
    \textbf{AF} & 33    & 45    & 77    & \textit{79} & 80    & \textcolor[rgb]{ 1,  0,  0}{\textbf{TBD}} \\
    \textbf{TRCE} & 16    & 48    & 133   & \textit{132} & 132   & \textcolor[rgb]{ 1,  0,  0}{\textbf{TBD}} \\
    \textbf{BUB} & 21    & 64    & 175   & \textit{174} & 174   & \textcolor[rgb]{ 1,  0,  0}{\textbf{TBD}} \\
    \textbf{CHN7} & 10    & 10    & 20    & \textit{20} & 20    & \textcolor[rgb]{ 1,  0,  0}{\textbf{TBD}} \\
    \textbf{CHN8} & 100   & 100   & 200   & \textit{200} & 200   & \textcolor[rgb]{ 1,  0,  0}{\textbf{TBD}} \\
    \textbf{CH2} & 4     & 8     & 10    & \textit{11} & 11    & \textcolor[rgb]{ 1,  0,  0}{\textbf{TBD}} \\
    \textbf{CH5} & 4     & 21    & 61    & \textit{53} & 71    & \textcolor[rgb]{ 1,  0,  0}{\textbf{TBD}} \\
    \textbf{GL2} & 25    & 50    & 56    & \textit{56} & 57    & \textcolor[rgb]{ 1,  0,  0}{\textbf{TBD}} \\
    \textbf{GL5} & 25    & 124   & 152   & \textit{147} & 155   & \textcolor[rgb]{ 1,  0,  0}{\textbf{TBD}} \\
    \textbf{GL10} & 25    & 249   & 323   & \textit{295} & 340   & \textcolor[rgb]{ 1,  0,  0}{\textbf{TBD}} \\
    \end{tabular}%
  \label{tab:benchmark_graph}%
  \caption{\small \textbf{Details of the benchmark graphs and the number of edges in the final contraction hierarchies for various algorithms.}}
\end{table}% 

==> teaser-full-table.tex <==
\begin{table}[t]
  \small
  \centering
    \begin{tabular}{c|c|ccc}
    \multicolumn{1}{c|}{\multirow{2}[1]{*}{Algorithms}} & \multicolumn{1}{c|}{\multirow{2}[1]{*}{Preprocess}} & \multicolumn{3}{c}{Query Distance Percentage} \\
    \multicolumn{1}{c|}{} &       & \multicolumn{1}{c}{1st} & \multicolumn{1}{c}{50th} & \multicolumn{1}{c}{99th} \\
    \midrule
    \multicolumn{1}{c|}{Dijkstra$^*$~\cite{dijkstra1959}} & -     & 0.468 s & 20.8 s & 42.0 s \\
    \multicolumn{1}{c|}{$\Delta$-stepping~\cite{dong2024pasgal}} & -     & 31.0 ms & 538 ms & 1180 ms \\
    \midrule
    \multicolumn{1}{c|}{RoutingKit$^*$~\cite{dibbelt2016customizable}} & 2466 s & 108 $\mu$s & 177 $\mu$s & 134 $\mu$s \\
    \multicolumn{1}{c|}{ch-constructor~\cite{??}} & 1527 s & 430 $\mu$s & 792 $\mu$s & 679 $\mu$s \\
    \multicolumn{1}{c|}{PHAST$^*$~\cite{delling2013phast}} & 1341 s & 259 $\mu$s & 353 $\mu$s & 224 $\mu$s \\
    Ours  & \textbf{23.1 s} & 153 $\mu$s & 220 $\mu$s & 165 $\mu$s \\
    \end{tabular}%
  \caption{\textbf{Preprocessing and query time on the road network of North America~\cite{roadgraph}.} (*) means sequential; others are parallel.
  1 $\mu$s = $10^{-6}$ s, and 1 ms = $10^{-3}$ s.
  The distance percentage of a query ($x$th) means the selected target is the $x$\% farthest vertex from each of the sources.
  CH algorithms are not sensitive to the query percentage.
  \xiaojun{Update the numbers for $\Delta$-stepping. Mention that Dijkstra is bidirectional.}}
  \label{tab:teaser_full}%
\end{table}%

